Using Processing Fluency as a Metric of Trust in Scatterplot Visualizations

Establishing trust with readers is an important first step in visual data communication. But what makes a visualization trustworthy? Psychology and behavioral economics research has found processing fluency (i.e., speed and accuracy of perceiving and processing a stimulus) is central to perceived trust. We examine the association between processing fluency and trust in visualizations through two empirical studies. In Experiment 1, we tested the effect of camouflaging a visualization on processing fluency. Participants estimated the proportion of data values within a specified range for six camouflaged visualizations and one non-camouflaged control; they also reported their perceived difficulty for each of the visualizations. Camouflaged visualizations produced less accurate estimations compared to the control. In Experiment 2, we created a decision task based on trust games adapted from behavioral economics. We asked participants to invest money in two hypothetical companies and report how much they trust each company. One company communicates its strategy with a camouflaged visualization, the other with a controlled visualization. Participants tended to invest less money in the company presenting a camouflaged visualization. Hence, we found support for the hypothesis that processing fluency is key to the perception of trust in visual data communication.

==> 02_RelatedWork.tex <==
% \section{Related Work}
% \label{relatedwork}

% Our work leverages theories and methods from psychology and behavioral economics to bridge existing explorations of trust in non-visual information communication with data visualization. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Trust in Non-Visualization Contexts}
% Existing research in communication, economics, and policy has revealed the difficulty of defining or measuring trust (e.g., \cite{gibson1998legitimacy, rudes2021legitimacy}). 
% The social sciences often measure trust via surveys that rely on participants' self-reports. These surveys prompt participants with questions such as ``generally speaking, would you say that most people can be trusted or that you need to be very careful in dealing with people?'' or ``on a scale from strongly agree to strongly disagree, how much do you trust this?'' \cite{naef2009measuring}.
% Nevertheless, quantifying trust is a complex task \cite{cho2015survey}. 
% To capture the complexity of trust, researchers have proposed additional trust measurements that examine its components. Self-reported perceived transparency, accuracy, clarity, amount of disclosure, and information thoroughness are positively associated with trust \cite{xiong2019examining, schnackenberg2016organizational}.

% However, the complexity and ambiguity of trust measurements \cite{schnackenberg2016organizational}, combined with the potential biases in self-reporting \cite{paulhus2007self}, have motivated researchers to explore alternative, more objective ways to measure trust. 
% A more modern method of measuring trust, particularly in the field of economics, is the Trust Game \cite{glaeser2000measuring, berg1995trust, zurn2017trust}. 
% In a typical trust game, two participants are anonymously paired. One participant is given an amount of money and told to send some money to the second participant (the amount may be zero). The experimenter takes the amount of money given and triples it before giving it to the second participant. The second participant must then send some money back to the first participant (the amount may be zero). Such trust games are a robust measure of trust, revealing how much each participant trusts the other; a larger money transfer indicates higher trust.
% Brülhart and Usunier \cite{brulhart2012does} support the robustness of the trust game by testing whether altruism or trust impact the results of the game; their experiment rejected altruism as a dominant factor in ``trust-like'' decisions.

% % Morrone et al. \cite{morrone2009how} describe standard methods for measuring interpersonal and institutional trust. Interpersonal trust is often measured using subjective reports via the Rosenberg question; Institutional trust is often measured using surveys asking individuals to rate subjective trust in several organizations. The relation between institutional and interpersonal trust is weak and, thus, one cannot be extrapolated to the other.


% \subsection{Trust in Visualizations}

% Perceived trustworthiness of visualizations and visualization systems also impacts how people conduct data analysis and make decisions \cite{honeycutt2020soliciting, nourani2019effects, hullman2011visualization, dork2013critical}. 
% For example, when scientists explore unfamiliar domains, they report model outputs communicated via a specialized tool that affords visualization and user interaction to be more trustworthy than analysis mediums such as Excel or MATLAB \cite{dasgupta2016familiarity}.
% In recent years, visualization researchers explore the effect of trust and methodologies to measure trust at the emerging workshop on trust and expertise in Visualization at IEEE (VIS TREX) \cite{nouraniwelcome}.

% Researchers have identified the volume and detail of information in visualizations as predictors of trust and perceived transparency \cite{hood2006transparency, xiong2019examining}. 
% Researchers found that the volume and detail of information predict trust and perceived transparency in visualizations \cite{kay2013there, jung2015displayed, joslyn2013}. 
% At the same time, too much information can overwhelm the viewer and distract from primary takeaways, leading to less interpretability \cite{sangdeh2021manipulating} and a decrease in trust \cite{kay2013there, jung2015displayed, joslyn2013}.
% Moreover, transparency without open discourse can ignore or undermine the communicative and reciprocal basis of trust \cite{moore2018towards, simmel1906sociology}. 


% High usability and a positive user experience can also enhance trust \cite{mayr2019trust, costante2011line, sasse2005usability}. 
% First impressions about the aesthetic design of websites, especially their colorfulness and complexity \cite{harrison2015infographic}, can impact the perceived usability and trustworthiness of the website, where more beautifully designed interfaces are perceived as more trustworthy  \cite{reinecke2013predicting}.
% However, when beautiful designs are coupled with highlighting and annotation, visualization readers may begin to question whether the visualization authors have an ulterior motive, leading to decreased trust \cite{ajani2021declutter}.
% Further, when presented with seemingly biased information, visualizations can be perceived as less credible \cite{kong2019trust}. 

% % Harrison et al. \cite{harrison2015infographic} studied first impressions of info-graphics and found that the mere exposure effect, colorfulness, and complexity impact how people create first impressions of info-graphics. They also found that the preferences in colorfulness and complexity varied with age, gender, and education level.
% % Considering the fact that first impressions about websites are made in the first few seconds of interaction and impact opinions of usability and trustworthiness, Reinecke et al. \cite{reinecke2013predicting} developed models to account for half of the variance in first-impressions (within 500ms) of a website.
% % 5Previous research has been done to measure trust in visualization. Xiong et al. \cite{xiong2019examining} found a link between individuals' ratings of transparency and ratings of trustworthiness of a visualization. The dimensions of transparency discussed in this paper include accuracy, clarity, amount of disclosure, and thoroughness. The paper concluded that subjective ratings of trust may not be effective in evaluating the trustworthiness of a visualization.
% % Mayr et al. \cite{mayr2019trust} describe the importance of trust in an individuals' likelihood to rely and build on information presented. This paper also mentions superficial cues as a possible metric indicating trustworthiness.
% % Dasgupta et al. \cite{dasgupta2016familiarity} measured the level of trust that scientists place in domain-specific visualizations and found that scientists were equivalently trustworthy of the visualizations despite a lack of knowledge of how the visualizations were created.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Processing Fluency}

% Processing fluency, which describes the subjective ease of perceiving or interpreting a stimuli, impacts human decision-making \cite{oppenheimer2008secret}.
% We can measure processing fluency by faster reaction time \cite{schooler2005forgetting}, higher self-reported satisfaction \cite{landwehr2020nature}, and lower self-reported difficulty when completing a task\cite{reber2004processing}.
% For example, Graf et al. \cite{graf2018measuring} found that a Likert scale ranging from self-reported ``difficult" to ``easy" is sufficient to measure processing fluency.
 
% Researchers have examined a variety of ways to manipulate processing fluency. 
% For example, people take longer to process and report less positive emotion with visual stimuli that are more complex, less clear, and more camouflaged, suggesting that visual complexity and camouflage are negatively associated with processing fluency \cite{flavell2020competing}.
% People also process aesthetically pleasing visual stimuli more fluently \cite{graf2015dual}, such as beautifully designed websites with the optimal amount of colorfulness and complexity \cite{harrison2015infographic}.
% For example, people report less satisfaction with stores that have more visually complex web pages \cite{sohn2017consumer}.
% The amount of exposure to a stimulus can also impact processing fluency, such that the longer exposure time and higher familiarity are positively associated with higher fluency \cite{mckean2020three, gordon1983implicit}.

% % \subsubsection{Processing Fluency and Aesthetics}
% % Labroo et al. \cite{labroo2008frog} found that priming people with a stimulus increased their experience of fluency with the stimulus later on. This effect was most present when using visual priming.
% % Graf et al. \cite{graf2015dual} developed the PIA model (Pleasure-Interest Model of Aesthetic Liking) which accounts for the aesthetic pleasure and aesthetic interest and their relation to fluent and dis-fluent stimuli. Previous research has found contradictory results regarding the impact of fluency on aesthetic liking, where some people would rate their aesthetic liking high for both fluent and dis-fluent stimuli. The PIA model accounts for this discrepancy by attributing aesthetic liking of a fluent stimuli to an aesthetic pleasure response and aesthetic liking of a dis-fluent stimuli to an aesthetic interest response.
% % \subsubsection{Processing Fluency and Affect}
% % Gordon and Holyoak \cite{gordon1983implicit} found that individuals preferred strings of characters that followed a grammar established by exposure to those that did not. This paper provides evidence that exposure impacts processing fluency positively.
% % Landwehr and Eckmann \cite{landwehr2020nature} presented five studies indicating that processing fluency has both a hedonic (positive affect increased) and amplification (both positive and negative affect amplified) effect on evaluative judgments of stimuli.


% % \subsection{Factors that increase Perceptual Fluency}
% % Flavell et al. \cite{flavell2020competing} tested reaction times with fluent and dis-fluent stimuli and found that fluent stimuli prompted faster reaction times. The methods of increasing and decreasing fluency presented in this paper include camouflage and contrast; camouflage refers to the addition of noise to a visual stimuli, contrast refers to the difference in value between the subject and background. This paper also found that more dis-fluency prompted higher rates of "liking" the stimulus.
% % McKean et al. \cite{mckean2020three} replicated the impact of processing fluency on immediate preference judgments. They also found that in situations where the measurement occurred after a longer period of time and a context-change (i.e. room change), processing fluency and inhibition only induced a preference change when combined.
% % Sohn \cite{sohn2017consumer} found that online stores with more perceived visual complexity were less fluent and lead to lower satisfaction, whereas stores with more perceived visual congruence were more fluent and lead to higher satisfaction.

% % Alter and Oppenheimer \cite{alter2009uniting} found a general ability to process fluency independent of the method used to generate the fluency. In other words, people judge perceptually fluent stimuli similarly to cognitively fluent or linguistically fluent stimuli.
% % Dech\^ene et al. \cite{dechene2010truth} compiled the results of 51 studies that test the truth effect via two methods: between-subjects (how much subjective truth ratings increase between repeated statements and other new statements) and within-subjects (how much subjective truth ratings increase from one encounter to the next of a single statement). The between-subjects truth effect was found to be larger than the within-subjects truth effect.
% % Graf et al. \cite{graf2018measuring}  tested a multi-item measure of processing fluency against a single-item measure. The paper found that both measures were able to account for five established fluency manipulations, and thus, the single-item measure (rating along a Likert scale from difficult to easy) is sufficient as an approach to measure processing fluency.


% \subsection{Processing Fluency and Trust}

% In a non-visual context, researchers have explored the positive association between processing fluency and trust \cite{schwarz2021metacognitive}. 
% In a trust game experiment comparing how people invest money in hypothetical investors with easier-to-pronounce or harder-to-pronounce usernames, researchers found that people were more likely to invest in (i.e., trust) those with easier-to-pronounce usernames \cite{zurn2017trust}.
% Researchers also found that people more easily process happy faces and subsequently trust happy faces more \cite{olszanowski2018mixed}.
% The present paper contributes to this literature by testing how we can manipulate processing fluency in data visualizations and measuring its effect on readers' perception of trust in the depicted data. 




==> Congruency_Stuff_that_was_originally_in_Section_6_backup.tex <==


%%%%% congruent stuff cut
\begin{comment}
Table \ref{odds2} shows the post-hoc analysis predicting accuracy with visualization display, congruency, and their interaction with using congruent bar reference. Note that because there were very few people who self-reported neutral attitude towards gun restriction laws, the corresponding statistics associated with neutral congruency were skewed to be either very large or very small. Generally, this supports our previous analysis that using the ratio strategy would boost accuracy. We see that even for bar displays, which generally yielded low accuracy, using the ratio strategy significantly improved the likelihood of a participant reaching the correct answer. 

\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.3} 
  \caption{Odds ratio of getting the correct answer by visualization design, belief congruency, and strategy used.}
  \begin{tabular}{llllll}
  \newline \\
    {\bf Variable} & {\bf Ratio} & {\bf Est}  & {\bf SE} & {\bf p-value}  & {\bf OR} \\
  \hline 
 congr. bars & no & -1.61 & 0.45 & 0.0032*** & 0.20\\
 neutral. bars & no & 0.63 & 0.81 &  0.44 & 1.88\\
 incongr. bars & no & -0.31 & 0.66 &  0.64 & 0.74\\
 congr. tables & no & 0.76 & 0.60 &  0.20 & 2.14 \\
 neutral. table & no & -17.35 & 1978 &  0.99 & 2.93e-08\\
 incongr. table & no & -0.84 & 0.98 &  0.39 & 0.44 \\
 congr. bars & yes & 1.79 & 0.75 &  0.017* & 6.00\\
 neutral. bars & yes & -18.38 & 3956 &  1.00 & 1.04e-08\\
 incongr. bars & yes &  0.41 & 1.17 &  0.73 & 1.51\\
 congr. table & yes & 0.22 & 0.99 & 0.83 & 1.24\\
 neutral. table & yes & 51.50 & 4845 &  0.99 & 2.32e+22\\
 incongr. table & yes & 0.96 & 1.61 &  0.55 & 2.60\\
    \end{tabular}
    \label{odds2}
\end{table}
\end{comment}
%%%%% congruent stuff cut

==> Old_Files/04_Exp1b.tex <==
\section{Experiment 1b}
The goal of Experiment 1b was to ensure that the low accuracy for the bar chart display condition in Experiment 1a, was not due the issues mentioned in the previous section. %misunderstandings of that those bars presenting percentages instead of counts. 
We redesigned the bar chart by adding gridlines, revising the row axis labels to clearly state that the bars reflected the \textit{number} of patients instead of a percentage, and increased the width of the bar marks to appear more similar to bars seen in typical designs, as shown in Figure \ref{teaser} (top right). %Experiment 1b modifies the bar display that has wider bars, gridlines, and axis labels, as shown in Figure \ref{teaser} (top right). %We are specifically interested whether this modified bar display would elicit different results from the one used in Experiment 1a. 

\subsection{Participants}
We recruited 85 participants on Mechanical Turk following the same procedure as Experiment 1a. Workers that completed Experiment 1a were not eligible to participate in Experiment 1b. All participants saw the revised bar chart, as shown in Figure \ref{teaser} (top right). % The exclusion criteria was the same as experiment 1a and we excluded 34 participants.%We excluded participants who spent less than 10 seconds reading the company prime story at the beginning (N = 19). Most of those participants who were excluded for spending less than 10 seconds on the company prime also wrote low-quality open ended responses (N=16). Additional participants were excluded from data analysis due to a low-quality open ended response (N = 4). Additional participants were excluded for missing 1 or more attention checks (N = 13). 
After excluding the participants following the same exclusion criteria as in Experiment 1, we ended up with 51 participants ($M_{age}$ = 18.86(10.90), 21 female).

% \subsection{Confidence Rating and Timing}
%[Elsie] Note to self: Add confidence and timing?

\subsection{Accuracy and Visualization Display Type}
We compare the accuracy for this second, modified bar chart display to the previous bar display from Experiment 1a. %\el{A $\chi^2$ test of independence with Bonferroni adjustment suggests the modified bars in Experiment 1b did not have a differing impact on decision task accuracy compared to the bars in Experiment 1a ($\chi^2$ = 0.90, $p$ = 0.34).} 
We conducted a comprehensive logistic regressions comparing the effect of display type (table, original bar, modified bar) on accuracy. We set the modified bar display as the baseline reference, and found it not significantly different from the bar display from Experiment 1a  ($Est = -0.46$, $SE = 0.40$, $p = 0.25$, $OR = 0.63$).
People who saw the modified bar chart did just as poorly on the reasoning task as those who saw the original bar chart.
Like the bar display from Experiment 1a, participants were less likely to make accurate judgments on skin cream effectiveness using this modified bar display compared to the table ($Est = 0.74$, $SE = 0.37$, $p = 0.047$, $OR = 2.11$). They were twice as likely to get the correct answer from the table display.

\subsection{Qualitative Coding}
The same coding structure was used from Experiment 1a. The qualitative responses were similar to the responses in Experiment 1a. 

\subsection{Strategy Analysis}
\label{1bStrategyAnalysis}
% which display used more ratio strategy?
In Experiment 1a, we have shown that participants were more likely to use the correct ratio strategy when they viewed the table compared to the bar chart. We explored whether the modified bar chart increased the likelihood of participants using the correct ratio strategy. We conducted a logistic regression comparing the odds ratio of participants using the ratio strategy between the modified bar chart, the original bar chart, and the tabular display, using the modified bar chart as reference. The model predicted whether participants used the ratio strategy with display type. People were just as unlikely to use the correct ratio strategy when they viewed the modified bar chart as when they viewed the original bar chart. ($Est = -0.56$, $SE = 0.39$, $p = 0.15$, $OR = 0.57$). They were significantly more likely to use the ratio strategy when they viewed the tabular display compared to the modified bar display ($Est =1.03$, $SE = 0.38$, $p = 0.0065$, $OR = 2.81$).

% how is using ratio strategy related to accuracy? 
We also examined the effect of display type and strategy used on accuracy. We constructed a logistic regression model predicting accuracy with display type (modified bar chart, original bar chart, and table), strategy (whether they used the correct ratio strategy or not), and their interaction. Once again, we found that accuracy is significantly driven by the strategy they used (${\chi}^2$ = 23.83, $p < 0.001$).

Table \ref{exp1b_OR} shows the likelihood of a participant answering the question correctly when they viewed a table, original bar chart, or modified bar chart, from left to right, respectively. The top row shows the likelihood of participants answering the reasoning question correctly when they do not use the ratio strategy. The bottom row shows how much using the ratio strategy would increase the likelihood of answering the question correctly for the three display types. For example, when participants viewed the tabular display, the odds of them answering the question correctly is 0.44. If they used the ratio strategy, those odds increase by 4.71 fold.

Interestingly, although participants were overall more likely to answer the questions correctly when they viewed the table (0.44 $>$ 0.28 and 0.44 $>$ 0.16, see \ref{exp1b_OR}), using the ratio strategy increases the odds of them answering the question correctly the most when they viewed the modified bar chart (13.39 $>$ 4.71 and 13.39 $>$ 2.40). The percentage of people that used the ratio strategy and answered the question correctly is similar in the table condition (33 answered correctly /49 total people that used the ratio strategy = 67\%) and the modified bar condition (33/49 = 68\%), more so than that in the original bar condition (8/20 = 40\%). The redesign of the bar chart appears to have improved performance slightly compared to the original design, but people still did not not nearly perform as well using the modified bar chart compared to the table.

% Can combine type label and center it between the two roles
% Cap first letter of cell
\begin{table}[!h]
       \small
    \caption{Likelihood of a participant answering correctly when viewing the three data display types, using or not using the ratio strategy. Each sub-table uses the no-ratio condition of that display type as the reference.}
    \begin{minipage}{.33\linewidth}
    \centering
          \begin{tabular}{llr}
  \newline \\
     \multicolumn{2}{c}{Table} \\
   {\bf Strategy} & {\bf OR} \\
  \hline 
 no & 0.44 \\
 ratio &  4.71 \\
     \end{tabular}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
        \centering
       \begin{tabular}{llr}
  \newline \\
   \multicolumn{2}{c}{Original Bars} \\
    {\bf Strategy} & {\bf OR} \\
  \hline
  no & 0.28 \\
 ratio &  2.40 \\
     \end{tabular}
    \end{minipage}
    \begin{minipage}{0.33\linewidth}
    \centering
       \begin{tabular}{llr}
    \newline \\     
     \multicolumn{2}{c}{Modified Bars} \\
  {\bf Strategy} & {\bf OR} \\
  \hline
  no &  0.16\\
 ratio &  13.39 \\
    \end{tabular}
    \end{minipage} 
        \label{exp1b_OR}
\end{table}

We compared three regression models, one with no predictors of accuracy, one with display type as a predictor, and one with display type and strategy both as predictors. We found that visualization display type significantly captures variances in the accuracy data ($Deviance = 11.87, p = 0.0026$), and additional consideration of strategy used during the reasoning task captures even more variances in the model ($Deviance = 27.56, p < 0.001$). 


%%%% Congruency section for completeness
\subsection{Congruency}
We again examined whether data-belief congruency affected accuracy, by constructing a logistic regression model predicting accuracy with display type (table, original bar chart, modified bar chart) and congruency (story prime congruent or incongruent with what the data suggests). Similar to Experiment 1a, we found a significant main effect of display type (${\chi}^2$ = 11.86, $p = 0.0027$) and a significant interaction of display type and congruency (${\chi}^2$ = 11.56, $p = 0.0031$). But no significant main effect of congruency ${\chi}^2$ = 0.145, $p = 0.70$).

More specifically, same as in Experiment 1a, people performed well when they viewed table displays, and were more likely to answer the question correctly when the data depicts a conclusion congruent with the story prime (e.g., effective skin cream, good company). But in Experiment 1a, although people performed poorly with bar charts, they were slightly better when their elicited belief is incongruent with the data. However, that was no longer the case with the modified bar chart. When participants viewed the modified bar chart, their performance was comparable when their belief is congruent and incongruent with the data. Table \ref{exp1b_congruency} shows the odds ratio comparison of the effect of congruency and display type on accuracy.

% edit table color
\begin{table}[!h]
 \small
    \caption{How does data-belief congruency affect accuracy for the three display types? The three table below shows the odds ratio of correctly answering the question. Left: Tabular display, with belief-data congruent condition as reference. Middle: Original bar chart, with the belief-data congruent condition as reference. Right: Modified Bar chart, with the belief data-congruent condition as reference.}
\begin{minipage}{.33\linewidth}
\centering
\begin{tabular}{lr}
  \newline \\
  \multicolumn{2}{c}{Table} \\
 {\bf Congruency} & {\bf OR} \\
  \hline 
 Congruent &  2.40\\
 Incongruent &  0.30 \\
     \end{tabular}
    \end{minipage}%
    \begin{minipage}{0.33\linewidth}
                             \centering
       \begin{tabular}{lr}
  \newline \\
     \multicolumn{2}{c}{Original Bars} \\
     {\bf Congruency} & {\bf OR} \\
  \hline
 Congruent & 0.15\\
 Incongruent &  4.14\\
     \end{tabular}
    \end{minipage}
    \begin{minipage}{0.33\linewidth}
                      \centering
       \begin{tabular}{lr}
    \newline \\     
        \multicolumn{2}{c}{Modified Bars} \\
        {\bf Congruency} & {\bf OR} \\
  \hline
 Congruent &  0.63\\
 Incongruent &  0.90 \\
    \end{tabular}
    \end{minipage} 
        \label{exp1b_congruency}
\end{table}

% Comparing the two bar displays, we see that participants were significantly more likely to give the correct answer for the \textit{congruent} condition when using modified bar display compared to the previous bar display. Although participants who viewed the modified bar displays in the congruent condition were less likely to get the answer correct compared to the participants who viewed the table display, we see from Figure \ref{results} that the likelihoods of participants getting the answer correct when they viewed the modified bar displays for the congruent and incongruent condition did not differ. This illustrated that primed belief did not have an effect on accuracy when participants viewed this modified display, suggesting that viewing the data via the modified bar display may be effective at mitigating confirmation bias. 


\subsection{Discussion} 
In Experiment 1B, \cx{people were not more likely (to a statistically reliable degree) to answer the question accurately, or to employ the correct ratio strategy, for the modified bar chart compared to the original condition in Experiment 1a}. % accuracy was not higher than for Experiment 1B.% participants overall were not more likely to respond correctly to the reasoning question when they viewed the bar charts in Exp 1B. 
\cx{People still performed better, and were more likely to use ratio strategies, for tabular displays compared to bar charts. People were not more likely to answer the question correctly when their story prime was congruent with the data. }
%Although for people who used the ratio strategy, more answered the correct when they viewed the modified bar chart than when they viewed the original bar chart. In other words, 
%the modified bar chart was an improvement compared to the original bar chart, both are still not as good as the tabular display.}

%\cx{While they were more likely to answer the questions correctly when their story prime is congruent with the data evidence when they viewed the table, it is unclear whether this data-belief congruency effect on accuracy exists only for tabular displays, or if it's driven by the story primes (experimenter demand effect). 
%In Experiment 2, we investigate a second scenario where people tend to have strong pre-existing beliefs - gun control legislation.}

%}There was also a similar rate of correct reasoning strategies. Participants who viewed the table designs still outperformed those that read the bar charts by using the correct ratio strategies more often.

%Overall accuracy for bars in experiment 1b was still far lower than the tabular condition, but was higher than the initial bar stimuli, although not significantly. Additionally, open-ended responses for the Exp 1B bar charts did not show higher accuracy compared to the Exp 1A bar charts. The addition of the gridlines also also appeared to push people to divide the bar charts into "units," and make calculations based on these units. One participant noted: "So in the figure A there were 9 units of people that got better and 3 units that got worse - or 1 person got worse for every 3 that got better. " Adding the grid lines allows people to more easily make judgements of magnitude. It also has the benefit of simplifying the larger numbers in the table to smaller, single digit units, although the abstract nature made it impossible to tell the absolute value of the bars. This suggests that the incorrect responses are due to the type of strategy used (heuristic) rather than an incorrect reading of the graph. %This reinforces the findings from Experiment 1a: the type of visual representation of bars is responsible for the difference in reasoning affordances. 

%Accuracy was the same between the congruent and incongruent conditions, suggesting that there was no confirmation bias for the bar graph display.

%We found a difference in congruent and incongruent conditions, but because we used a prime, we decided to test the same task, but with pre-existing beliefs instead of primed beliefs.


%We explored whether the modified bar displays were more likely to elicit ratio strategies, by comparing the odds ratio to the bar and table displays from Experiment 1a. We used a logistic regression model predicting strategy using the modified bar display as the baseline reference. We found that \textbf{people were just as unlikely to use the correct ratio strategy when they viewed the modified bar chart as when they viewed the original bar chart.} ($Est = -0.56$, $SE = 0.39$, $p = 0.15$, $OR = 0.57$). They were still more likely to use the ratio strategy when they viewed the table display compared to the modified bar display ($Est = 1.03$, $SE = 0.38$, $p = 0.0065$, $OR = 2.81$). 

% Again, viewers were more likely to use the ratio strategy when viewing the data in tabular displays ($Est = 1.03, SE = 0.38, p = 0.006$), although we observed a decrease in effect size ($OR = 2.80$) such that tabular displays only increased the odds ratio of participants using the ratio strategy by around three fold. 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\begin{comment}
\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.3}
  \caption{Participants who viewed the tabular display and used the ratio strategy were more likely to get the answer correct.}
  \begin{tabular}{llr}
  \newline \\
    {\bf Display} & {\bf Strategy}  & {\bf Odds Ratio for Accuracy} \\
  \hline 
 exp1 table  & no ratio &  2.73  \\
 modified bar & no ratio & 0.16 \\
 exp1 bar & no ratio & 1.74 \\
 
 modified bar  & ratio &  13.39  \\
 exp1 bar & ratio & 0.18 \\
 exp1 table  & ratio &  0.35  \\
    \end{tabular}
    \label{exp1b_OR}
\end{table}

\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.3}
  \caption{How much does the new modified bar display increase the odds ratio of getting the correct answer compared to the displays from Experiment 1?}
  \begin{tabular}{llr}
  \newline \\
    {\bf Display} & {\bf Congruency} & {\bf Odds Ratio} \\
  \hline 
 bar & congruent &  -0.25 \\
 bar & incongruent &  1.13 \\
 table & congruent & 3.84 \\
 table & incongruent &  1.29 \\
    \end{tabular}
    \label{oddsbar2}
\end{table}
\end{comment}

==> Old_Files/Old_Confirmation_Bias_Text.tex <==

% Confirmation bias is the tendency to search for information that supports prior beliefs, and drawing conclusions without considering information that may suggest otherwise. This bias affects people throughout the information gathering process, from what people selectively search for, focus on, remember information, to ultimately what information they use to make decisions \cite{Wason1968Rule, Nickerson1998}. This bias could occur in many contexts, from selectively reading articles online to ignoring your coworker who has different beliefs than you. 

% An example display of data that has been shown to induce bias is in figure \ref{teaser}a. \cx{Add a description of what Figure 1a is showing - specifically, the number represents the # cities that experienced an increase/decrease in crime. In the figure caption or here. Too confusing right now.} Using the table, answer the question, "Did banning carrying concealed handguns in public increase or decrease crime?" Depending on people's prior belief about gun-control laws, they tend to focus on different data patterns in the table \cite{Kahan2017Motivated} depicted in (a). \cx{A person who thinks gun-control laws are critical to reduce crime would pay attention to ... and conclude.... A person who is against gun-control laws woud.... -> explicitly illustrate the confirmation bias here. }To get the correct answer, you should compare the proportion of crime increases and decreases under different circumstances. Looking at the top row, crime decreases in 25\% of the cities that banned concealed carry (75/(223+75)), but only decreased in 16\% of the cities that did not ban concealed carry (21/(107+21)), as shown in the bottom row. For these particular data, once normalized with this strategy of converting numbers to ratios, it is clear that the ban is associated with reductions in crime. 


% Kind of describing this backwards from what we imagine is going on. First you see the quick heuristic, then you try to do the ratio strategy

% But for most people, that is a tough analytic task, requiring them to compare two ratios between pairs of numbers. It is tempting to use faster heuristics to interpret this data, which can lead to systematic biases \cite{kahneman1982}. If they don't believe that a ban would decrease crime, they would be motivated to use the data to come to a conclusion that is in line with their prior beliefs. Some people believe that banning concealed handguns will actually \textit{increase} crime, by removing a deterrent to criminal behavior. To do this, they could focus on only the top row of the data. For cities that banned concealed carry, crime increased in 223 cities, which is a lot more than the 75 cities that had a decrease in crime. This difficult task allows people to see the data from multiple perspectives which might justify either conclusion. These diverging conclusions illustrate confirmation bias. \cx{Move this section to where I noted to explicitly illustrate CB - it follows your point on "they tend to focus on diferent data patterns in the table" nicely.}


%But, what would happen if this same data was visualized in a graphical display? Would people still have a bias to search for and interpret patterns that confirm their prior beliefs? In visualizations, people might similarly succumb to confirmation bias, searching for patterns and trends in a graph that supports their beliefs, while missing patterns and trends that contradict their beliefs. However, the visual display of the graph might make it harder to ignore patterns that they don't agree with. If so, confirmation bias would be reduced.


% What is confirmation bias and how does it work?
% Framing hypotheses to confirm
%One classic task that demonstrates confirmation bias is the Wason Card selection task \cite{Wason1968Rule}. There are four cards that each have a number or letter on the front: a vowel, a consonant, an even number, or an odd number (e.g. A, B, 4, and 7). The task is to choose which cards to flip over in order to determine the veracity of the statement: ``If there is a vowel on one side of the card, then there is an even number on the other side''. People readily chose A, because if there was an even number on the other side, this card would confirm the previous statement. Fewer people chose to flip over the odd numbered card, which could also falsify the statement if it had a vowel on the other side. This is an example of confirmation bias, because people seek out information to confirm, but not to disconfirm, the original statement. 

%Confirmation bias has been studied through various experiments in psychology, but it is prevalent in real world applications as well. For example, a person who dislikes guns may search on the internet ``will gun control laws decrease crime?" This query is phrased to seek out information to confirm their belief. If this person was actively trying to seek out information opposite to their beliefs, they could have searched ''does concealed carry reduce crime?" In another example, people are more likely to frame hypotheses in a way that would affirm if a person was suited for the job, rather than unsuited \cite{Snyder1979Jane}. 

% Ignoring information
%Another way that confirmation bias affects the information gathering process is that people will ignore results that do not align with their prior beliefs. For example, this person's top result is "These Gun Laws Can Actually Reduce Gun Deaths", but the third result is "Crime, Deterrence, and Right-to-Carry Concealed Handguns". If they only read the results that are congruent with their prior beliefs and conveniently ignore any titles that suggest opposing information, this would be confirmation bias. On social media, people are more likely to follow people who share similar beliefs, rather than follow those who hold opposing beliefs. This can create a filter bubble, where users are only exposed to ideas that they already agree with \cite{pariser2011filter}. 

%Favoring information
%Perhaps this person did read both positive and negative information about concealed carry gun laws. If they favored the information on stricter restrictions on guns and disregarded the information that they didn't agree with, then that is another way that confirmation bias affects decisions.

%Confirmation bias can affect people every day, from small beliefs such as ''coffee is good for you" to much more important issues such as ''banning concealed carry will decrease crime." Confirmation bias may not have serious ramifications for drinking coffee, but gathering information about important decisions such as vaccinations, health risks, medical decisions, could have serious implications not just for the person making the decision, but also the community around the person. 
\cx{I don't think you need to argue for the use of MTurk. Quality of workers on this platform is comparable to other traditional subject pools \cite{Paolacci2010, buhrmester2016amazon}. Nevertheless, }
% Using a decision task established in the psychology literature showing interpretation of data presented in a table format could invite confirmation bias \cite{Kahan2017Motivated}, this paper investigates whether visualizing the same information with a bar graph could mitigate this bias. We used a between-subject design for the experiments to examine the effect of data display type and prior belief on decisions. 

\subsubsection{Mechanical Turk}
We recruited participants for our experiments through Amazon Mechanical Turk. This platform allows us to recruit a larger number of participants than an in-person sample, which was essential for this between-subjects design. Additionally, Mechanical Turk has been argued to be a more realistic setting for real-life decision making tasks than an undergraduate university setting \cite{Micallef2012}. In order to qualify for our study, participants needed to have a 95\% acceptance rate and to be located in the United States. 

Quality of workers on this platform is comparable to other traditional subject pools \cite{Paolacci2010, buhrmester2016amazon}. Nevertheless, we implemented a series of quality checks to ensure that workers were paying attention (e.g., ``How many years of experience of Computer Programming do you have? Please choose "10+"  to show that you are paying attention.''). In addition to these traditional attention check multiple choice questions, we were able to track through Qualtrics how long a person stayed on a page. We used this to filter out workers who spent less than 10 seconds reading the descriptions of company, which was 2 paragraphs long. 

Another check for quality was our open ended responses. These may have been the most obvious to check for people that were not putting in effort into the survey. Low-quality responses ranged from off topic answers to intelligible sentences. Often, the workers who failed the timing check also failed the open-ended response check, suggesting that these two measures were both catching people who were not paying attention. \el{I think there was something (a paper? a website?) that mentioned using open ended responses for checking MTurkers, but I just searched and couldn't find it again}

\subsubsection{Participants}

We collected data from 218 participants on Amazon Mechanical Turk. We asked workers to self-report their demographic information.

\el{Elsie add demographics?}


\cx{repetitive, cut}
% \subsection{Results}
% In order to filter out Mechanical Turk workers who were not paying attention, we implemented a series of criteria for excluding participants from data analysis. We excluded participants who spent less than 10 seconds reading the company prime story at the beginning (N=30). Most participants who spent less than 10 seconds reading the company prime story also wrote low quality open ended responses (N=18). Additional participants were also excluded for low quality open ended responses (N=19). Additional participants were excluded for missing one or more attention checks (N = 31). The resulting data analyzed was from 138 participants. 


Prior beliefs and group identities influence how people interpret data about politically-charged topics, presented in tables \cite{Kahan2017Motivated}. Those participants were shown a 2x2 contingency table of data on gun control laws as shown in Figure \ref{teaser}a. Participants then decided whether the gun control laws were more likely to be associated with an \textit{increase} or \textit{decrease} in crime. This experiment also contained a neutral condition where participants viewed the same table but it was re-framed as skin-cream effectiveness (Figure \ref{stimuli}a), intended to serve as a baseline measure of analytic ability in the absence of cognitive bias. In experiment 1, we adapt this neutral skin-cream condition to investigate if the bias would still occur with a primed belief rather than an existing one.  \cx{how is the 2x2 table we present different from a Bayesian reasoning problem? Are they the same? If so, what is our motivation of not calling it a bayesian problem? The Bayesian ppl in the vis community that would probably want some clarification.}

==> Old_Files/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Old_Files/garbage.tex <==
%%%  INTRODUCTION  %%%

% Example of teaser image
An example display of data that has been shown to have multiple interpretations is in figure \ref{teaser}a. Using the table, answer the question, "Did banning carrying concealed handguns in public increase or decrease crime?" Depending on people's prior belief about gun-control laws, they tend to focus on different data patterns in the table \cite{Kahan2017Motivated} depicted in (a). 

%Heuristic
A person who thinks concealed carry guns are a deterrent to reduce crime might notice that there were 223 cities that did \textbf{ban} carrying concealed handguns in public that had an increase in crime. That's a lot of cities, way more than the 75 cities that had a decrease in crime. This person might conclude that if cities ban concealed carry, crime will increase. This is actually a quick heuristic strategy, which only focuses on the top row and ignores half of the data.

%Ratio
On the other hand, some people believe that banning concealed handguns will actually \textit{increase} crime, by removing a deterrent to criminal behavior. A person like this might look at this same data and come to a different conclusion. They might instead compare the proportion of crime increases and decreases under different circumstances. Looking at the top row, crime decreases in 25\% of the cities that banned concealed carry (75/(223+75)), but only decreased in 16\% of the cities that did not ban concealed carry (21/(107+21)), as shown in the bottom row. For these particular data, once normalized with this “ratio” strategy of converting numbers to ratios, it is clear that the ban is associated with reductions in crime. 

%Discussion of two strategies
However, for most people, this ratio strategy is a tough analytic task, requiring them to compare two ratios between pairs of numbers. When people care less about finding the correct answer, they use faster heuristics to interpret this data, which can lead to systematic biases \cite{kahneman1982}. This difficult task allows people to use different reasoning strategies to see the data from multiple perspectives.

% Study Motivation

In this paper, we are interested in looking at the different reasoning affordances for data displays, and how these affect the prevalence of “heuristic” and “ratio” strategies in our task.

% Different Reasoning Systems / Systems 1 and 2
% Why Data Visualization is Powerful

% Study Overview 

Across two experiments, we use an established Psychology task to investigate reasoning affordances in tables and bar charts. With a 2x2 data display, people can interpret the data in multiple ways, either using a quick heuristic or a slower “ratio” strategy. 

We first used a neutral topic of skin cream with a primed belief about the efficacy of the skin cream to test these different strategies. We then explored how the same task with a polarizing topic of gun control could influence reasoning affordances.

Our findings show that bar graphs led to a strong preference for using the heuristic strategy. 
%Experiment 1 suggested that the primed beliefs replicated a bias effect in the table condition. We examined their strategies in more detail to further understand the reasoning affordances for tables and bar graphs. Finally, we consider future directions for how reasoning affordances intersect cognitive biases and how visualizations could mitigate these biases.


\section{Reasoning Systems}

%Discussion of System 1 and System 2

There are two systems of thinking in the brain. Most of the time, we use system 1 thinking, which is faster and relies on heuristics. This is also where cognitive biases come into play.

%System 2
On the other hand, system 2 thinking is slower, more “rational”, but also takes a lot more cognitive effort.

\section{Visualizations}

%Why visualization can be a good mitigation
In this study, we are interested in studying whether or not visualizations would affect reasoning patterns in a tabular display. If data is instead visualized, would this make it harder or easier to ignore patterns that do not align with your previous beliefs? If a pattern is easy to see and salient, it could be harder to discount it, even if you disagree with it. On the other hand, if a pattern is difficult to see, it could be easier to ignore it. 

% \cx{Present this section as a hypothesis that could go either way - could we mitigate confirmation bias with visualizations? \textbf{Maybe Yes} - because visualizations help. (Cite \cite{larkin1987diagram}, which suggests effective visualization designs can offload cognitive work to the perceptual system, and more effectively communicating information in an accessible and interpretable way; cite the 2x2 table studies suggesting that visualizations help; also cite Dimara 2019, Mitigating the Attraction Effect with Visualizations; cite Improving Bayesian reasoning: The effects of phrasing, visualization,and spatial ability by ottley/harrison 2016, showing that pictographs and isotypes help communicate bayesian reasoning) \textbf{Maybe No} - because visualization highlight different patterns (cite my curse stuff), motivated perception - patterns congruent to belief are looked at more/appear more salient (cite Luo and Zhao, 2019, Motivated attention in climate change perception and action), decisions are driven by personal experience when ppl look at visualizations (cite Data is Personal: Attitudes and Perceptions of Data Visualization in Rural Pennsylvania, peck, ayuso et al.) }

But, what would happen if this same data was visualized in a graphical display? What types of reasoning people do - heuristics or slower ratio? In visualizations, people might similarly rely on heuristics, searching for patterns and trends in a graph that are easy to see, while missing patterns and trends that take longer to see. However, the visual display of the graph might make it harder to ignore patterns that they don't agree with. If so, confirmation bias would be reduced.

Visual processing allows patterns to be seen quickly and easily.
\el{Cindy/Steve - would you suggest any papers I should cite?}
\cx{steal sections from my Curse of knowledge OPAM submission (not archived), attached below:}

\cx{The visual system seeks meaning in the image presented by the world, by matching visual input to hypotheses about object identities and spatial relations. Sometimes, as demonstrated in the duck-rabbit and Necker cube illusions, multiple hypotheses might exist (Attneave, 1971), leading two people having different interpretations of the same image. While such ambiguity is actually rare in the natural world, it is ubiquitous in the artificial world of information visualizations. A graph, for example, contains many potential perceivable patterns. After viewers extract a set of ensemble statistics about the dataset (Szafir et al., 2016), they must exercise top-down attentional control (Egeth et al., 2010) to extract a series of relationships and patterns from the data values (Michal et al., 2016; 2017), with an equivalent time and effort to reading a paragraph (Shah and Freedman, 2011). The diversity of percepts extractable from patterns in graphs might lead to two people seeing different patterns in the same graph - one the 'duck' and the other the 'rabbit'. The curse of knowledge experiment shows that top-down cues (a verbal description of a particular pattern) can increase visual salience for that particular pattern, driving it so strongly that participants could not turn it 'off'. After giving a verbal description of a particular pattern, we asked participants to imagine the graph from a naive perceptive, as when they first saw it, and to predict what a naive viewer would find salient. Participants could not recover an unbiased percept of the image, and they strongly predicted that others would see the same newfound salience that they saw.}

\el{Discussion on informational equivalence vs computational equivalence?}
\cx{not sure what this means}


\subsection{Hypotheses}

Could we mitigate confirmation bias with visualizations? \textbf{Maybe Yes} - because visualizations help. (Cite \cite{larkin1987diagram}, which suggests effective visualization designs can offload cognitive work to the perceptual system, and more effectively communicating information in an accessible and interpretable way; cite the 2x2 table studies suggesting that visualizations help; also cite Dimara 2019, Mitigating the Attraction Effect with Visualizations; cite Improving Bayesian reasoning: The eects of phrasing, visualization,and spatial ability by ottley/harrison 2016, showing that pictographs and isotypes help communicate bayesian reasoning) \textbf{Maybe No} - because visualization highlight different patterns (cite my curse stuff), motivated perception - patterns congruent to belief are looked at more/appear more salient (cite Luo and Zhao, 2019, Motivated attention in climate change perception and action), decisions are driven by personal experience when ppl look at visualizations (cite Data is Personal: Attitudes and Perceptions of Data Visualization in Rural Pennsylvania, peck, ayuso et al.) 

%Examples of visualization tools // relevant work

Cognitive biases are becoming a topic of interest in the visualization community \cite{Dimara2018Taxonomy, Ellis2015, Wall2019}, and visualization tools have been developed to help people overcome cognitive biases. \cx{previously you zoomed-in and specifically talked about CB, it reads weird now that you are zooming out to talk about cognitive biases as a whole. Reverse the sections, or maybe reframe this section to discuss mitigation of cognitive biases using visualization tools.}
In a highly-subjective process like college admission reviews, biases such as availability bias, representativeness, anchoring, confirmation bias, could be mitigated by presenting data in visualizations to encourage multiple interpretations of the data \cite{Sukumar2018}. 
For analytical tasks that involve using many pieces of evidence, Sandbox is a software tool that allows users to visually organize information to reduce cognitive biases and increase performance \cite{Wright2006Sandbox}. This software encourages users to explore multiple hypotheses and record supporting or rejecting evidence when working with data \cite{Wright2006Sandbox}. 
Another application is JIGSAW - Joint Intelligence Graphical Situation Awareness Web, which uses a graphical evidence layout to help reduce bias in tactical decision making \cite{Cook2008, Smallman2017}. 
%Wall \cite{Wall2019} explores the space of how design spaces could be created to help promote less-biased decision making. %added cite for Wall above
\cx{cite Wall's short paper on mitigaing Cognitive bias - Towards a Design Space for Mitigating Cognitive Bias in Visual Analytics, 2020; maybe cite  Bancilhon et al on risk perception and decision making with visualizations - Let's Gamble: Uncovering the Impact of Visualization on Risk Perception and Decision-Making}



%Visualizations and Medical decision making
Visualizations have improved understanding of complicated data in the medical decision making field as well, where biases such as framing \cx{which is?} or base-rate neglect \cx{which is} can affect decisions. Tables, tree diagrams \cite{Binder2015}, or pictographs \cite{Tait2010} improve comprehension of data compared to text. Displaying data in a bar graph increased comprehension of efficacy of a drug compared to text \cite{Dragicevic2017}. Interestingly, this study also showed that prior belief in science predicted the perceived efficacy of the drug. Additionally, the authors argue that in order to study the effects of biases from the visualizations, comprehension of data from visualized data needs to be analyzed as well \cite{Dragicevic2017}. However, not all complicated decisions are helped by adding visualizations. In a difficult Bayesian problem, adding Euler diagrams or frequency grids did not improve performance over just text \cite{Micallef2012}. 

% Confirmation Bias has been shown to occur in Kahan
System 1 and System 2 thinking comes into play with an example of Motivated Reasoning with the table shown in \ref{teaser}a. 
 
Prior beliefs and group identities influence how people interpret data about politically-charged topics, presented in tables \cite{Kahan2017Motivated}. Those participants were shown a 2x2 contingency table of data on gun control laws as shown in Figure \ref{teaser}a. Participants then decided whether the gun control laws were more likely to be associated with an \textit{increase} or \textit{decrease} in crime. This experiment also contained a neutral condition where participants viewed the same table but it was re-framed as skin-cream effectiveness (Figure \ref{stimuli}a), intended to serve as a baseline measure of analytic ability in the absence of cognitive bias. In experiment 1, we adapt this neutral skin-cream condition to investigate if the bias would still occur with a primed belief rather than an existing one.  \cx{how is the 2x2 table we present different from a Bayesian reasoning problem? Are they the same? If so, what is our motivation of not calling it a bayesian problem? The Bayesian ppl in the vis community that would probably want some clarification.} \el{Ok, how do we talk about it in a Bayesian way? I’m not very familiar with the area.}


\subsection{Contributions} 
One contribution of this work is to test whether the new participant-priming version of the skin cream example could replicate the type of confirmation bias found in past work for topics where participants had existing opinions (e.g. the efficacy of gun control laws). A replication would provide a methodologically important contribution, removing the need to selectively recruit participants with particular views on a tested topic. 


An example display of data that has been shown to have multiple interpretations is in figure \ref{teaser}a. Using the table, answer the question, "Did banning carrying concealed handguns in public increase or decrease crime?" Depending on people's prior belief about gun-control laws, they tend to focus on different data patterns in the table \cite{Kahan2017Motivated} depicted in (a). 
A person who thinks concealed carry guns are a deterrent to reduce crime might notice that there were 223 cities that did \textbf{ban} carrying concealed handguns in public that had an increase in crime. That's a lot of cities, way more than the 75 cities that had a decrease in crime. This person might conclude that if cities ban concealed carry, crime will increase.
On the other hand, some people believe that banning concealed handguns will actually \textit{increase} crime, by removing a deterrent to criminal behavior. A person like this might look at this same data and come to a different conclusion. They might instead compare the proportion of crime increases and decreases under different circumstances. Looking at the top row, crime decreases in 25\% of the cities that banned concealed carry (75/(223+75)), but only decreased in 16\% of the cities that did not ban concealed carry (21/(107+21)), as shown in the bottom row. For these particular data, once normalized with this strategy of converting numbers to ratios, it is clear that the ban is associated with reductions in crime. 

However, for most people, that is a tough analytic task, requiring them to compare two ratios between pairs of numbers. It is tempting to use faster heuristics to interpret this data, which can lead to systematic biases \cite{kahneman1982}.  
This difficult task allows people to see the data from multiple perspectives which might justify either conclusion. These diverging conclusions illustrate confirmation bias.


% \cx{Present this section as a hypothesis that could go either way - could we mitigate confirmation bias with visualizations? \textbf{Maybe Yes} - because visualizations help. (Cite \cite{larkin1987diagram}, which suggests effective visualization designs can offload cognitive work to the perceptual system, and more effectively communicating information in an accessible and interpretable way; cite the 2x2 table studies suggesting that visualizations help; also cite Dimara 2019, Mitigating the Attraction Effect with Visualizations; cite Improving Bayesian reasoning: The eects of phrasing, visualization,and spatial ability by ottley/harrison 2016, showing that pictographs and isotypes help communicate bayesian reasoning) \textbf{Maybe No} - because visualization highlight different patterns (cite my curse stuff), motivated perception - patterns congruent to belief are looked at more/appear more salient (cite Luo and Zhao, 2019, Motivated attention in climate change perception and action), decisions are driven by personal experience when ppl look at visualizations (cite Data is Personal: Attitudes and Perceptions of Data Visualization in Rural Pennsylvania, peck, ayuso et al.) }

But, what would happen if this same data was visualized in a graphical display? What types of reasoning people do - heuristics or slower ratio? In visualizations, people might similarly rely on heuristics, searching for patterns and trends in a graph that are easy to see, while missing patterns and trends that take longer to see. However, the visual display of the graph might make it harder to ignore patterns that they don't agree with. If so, confirmation bias would be reduced.


% Study Overview 

Across two experiments, we use an established Psychology task to investigate reasoning affordances in tables and visualized data. With a 2x2 table, people can interpret the data in multiple ways, either using a quick heuristic or a slower rational reasoning. 

We first used a neutral topic of skin cream to test these different reasoning affordances. We then explored how the same task with a polarizing topic of gun control could influence reasoning affordances.

Our findings show that people are more likely to use a heuristic strategy when interpreting visualized data.

We empirically test the strength of confirmation bias in tabular and bar charts  We first constructed a novel tabular data example where we primed beliefs, instead of relying on existing beliefs, and replicated a bias effect. We then created a version with simple visualizations (bar graphs), and were surprised to find that the bar graphs led to a strong preference for using the heuristic strategy \cx{which is?}. Additionally, we tested this bias on a topic that people have prior beliefs on (gun control laws) and found the same findings \cx{replicated CB in table, not in bars}. We hypothesize why this may be and consider future directions for researching visualizations for mitigating biases \cx{reframe as we dove deeped by examining their strategies, which suggested that they were using heuristics...}

\section{Background}


%Why visualization can be a good mitigation
In this study, we are interested in studying whether or not visualizations would affect reasoning patterns in a tabular display. If data is instead visualized, would this make it harder or easier to ignore patterns that do not align with your previous beliefs? If a pattern is easy to see and salient, it could be harder to discount it, even if you disagree with it. On the other hand, if a pattern is difficult to see, it could be easier to ignore it. 

Visual processing allows patterns to be seen quickly and easily.
\el{Cindy/Steve - would you suggest any papers I should cite?}
\cx{steal sections from my Curse of knowledge OPAM submission (not archived), attached below:}

\cx{The visual system seeks meaning in the image presented by the world, by matching visual input to hypotheses about object identities and spatial relations. Sometimes, as demonstrated in the duck-rabbit and Necker cube illusions, multiple hypotheses might exist (Attneave, 1971), leading two people having different interpretations of the same image. While such ambiguity is actually rare in the natural world, it is ubiquitous in the artificial world of information visualizations. A graph, for example, contains many potential perceivable patterns. After viewers extract a set of ensemble statistics about the dataset (Szafir et al., 2016), they must exercise top-down attentional control (Egeth et al., 2010) to extract a series of relationships and patterns from the data values (Michal et al., 2016; 2017), with an equivalent time and effort to reading a paragraph (Shah and Freedman, 2011). The diversity of percepts extractable from patterns in graphs might lead to two people seeing different patterns in the same graph - one the 'duck' and the other the 'rabbit'. The curse of knowledge experiment shows that top-down cues (a verbal description of a particular pattern) can increase visual salience for that particular pattern, driving it so strongly that participants could not turn it 'off'. After giving a verbal description of a particular pattern, we asked participants to imagine the graph from a naive perceptive, as when they first saw it, and to predict what a naive viewer would find salient. Participants could not recover an unbiased percept of the image, and they strongly predicted that others would see the same newfound salience that they saw.}

\el{Discussion on informational equivalence vs computational equivalence?}
\cx{not sure what this means}

\subsection{Related Work}

Could we mitigate confirmation bias with visualizations? \textbf{Maybe Yes} - because visualizations help. (Cite \cite{larkin1987diagram}, which suggests effective visualization designs can offload cognitive work to the perceptual system, and more effectively communicating information in an accessible and interpretable way; cite the 2x2 table studies suggesting that visualizations help; also cite Dimara 2019, Mitigating the Attraction Effect with Visualizations; cite Improving Bayesian reasoning: The eects of phrasing, visualization,and spatial ability by ottley/harrison 2016, showing that pictographs and isotypes help communicate bayesian reasoning) \textbf{Maybe No} - because visualization highlight different patterns (cite my curse stuff), motivated perception - patterns congruent to belief are looked at more/appear more salient (cite Luo and Zhao, 2019, Motivated attention in climate change perception and action), decisions are driven by personal experience when ppl look at visualizations (cite Data is Personal: Attitudes and Perceptions of Data Visualization in Rural Pennsylvania, peck, ayuso et al.) 

%Examples of visualization tools // relevant work
Cognitive biases are becoming a topic of interest in the visualization community \cite{Dimara2018Taxonomy, Ellis2015, Wall2019}, and visualization tools have been developed to help people overcome cognitive biases. \cx{previously you zoomed-in and specifically talked about CB, it reads weird now that you are zooming out to talk about cognitive biases as a whole. Reverse the sections, or maybe reframe this section to discuss mitigation of cognitive biases using visualization tools.}
In a highly-subjective process like college admission reviews, biases such as availability bias, representativeness, anchoring, confirmation bias, could be mitigated by presenting data in visualizations to encourage multiple interpretations of the data \cite{Sukumar2018}. 
For analytical tasks that involve using many pieces of evidence, Sandbox is a software tool that allows users to visually organize information to reduce cognitive biases and increase performance \cite{Wright2006Sandbox}. This software encourages users to explore multiple hypotheses and record supporting or rejecting evidence when working with data \cite{Wright2006Sandbox}. 
Another application is JIGSAW - Joint Intelligence Graphical Situation Awareness Web, which uses a graphical evidence layout to help reduce bias in tactical decision making \cite{Cook2008, Smallman2017}. 
%Wall \cite{Wall2019} explores the space of how design spaces could be created to help promote less-biased decision making. %added cite for Wall above
\cx{cite Wall's short paper on mitigaing Cognitive bias - Towards a Design Space for Mitigating Cognitive Bias in Visual Analytics, 2020; maybe cite  Bancilhon et al on risk perception and decision making with visualizations - Let's Gamble: Uncovering the Impact of Visualization on Risk Perception and Decision-Making}

%Visualizations and Medical decision making
Visualizations have improved understanding of complicated data in the medical decision making field as well, where biases such as framing \cx{which is?} or base-rate neglect \cx{which is} can affect decisions. Tables, tree diagrams \cite{Binder2015}, or pictographs \cite{Tait2010} improve comprehension of data compared to text. Displaying data in a bar graph increased comprehension of efficacy of a drug compared to text \cite{Dragicevic2017}. Interestingly, this study also showed that prior belief in science predicted the perceived efficacy of the drug. Additionally, the authors argue that in order to study the effects of biases from the visualizations, comprehension of data from visualized data needs to be analyzed as well \cite{Dragicevic2017}. However, not all complicated decisions are helped by adding visualizations. In a difficult Bayesian problem, adding Euler diagrams or frequency grids did not improve performance over just text \cite{Micallef2012}. 

% Confirmation Bias has been shown to occur in Kahan
Prior beliefs and group identities influence how people interpret data about politically-charged topics, presented in tables \cite{Kahan2017Motivated}. Those participants were shown a 2x2 contingency table of data on gun control laws as shown in Figure \ref{teaser}a. Participants then decided whether the gun control laws were more likely to be associated with an \textit{increase} or \textit{decrease} in crime. This experiment also contained a neutral condition where participants viewed the same table but it was re-framed as skin-cream effectiveness (Figure \ref{stimuli}a), intended to serve as a baseline measure of analytic ability in the absence of cognitive bias. In experiment 1, we adapt this neutral skin-cream condition to investigate if the bias would still occur with a primed belief rather than an existing one.  \cx{how is the 2x2 table we present different from a Bayesian reasoning problem? Are they the same? If so, what is our motivation of not calling it a bayesian problem? The Bayesian ppl in the vis community that would probably want some clarification.}

\subsection{Contributions} 
One contribution of this work is to test whether the new participant-priming version of the skin cream example could replicate the type of confirmation bias found in past work for topics where participants had existing opinions (e.g. the efficacy of gun control laws). A replication would provide a methodologically important contribution, removing the need to selectively recruit participants with particular views on a tested topic. 

%INTRODUCTION

%Example of the Teaser Image
Based on the data presented in \ref{teaser}, does the skin cream make rashes worse or better? 

%Example Heuristic Strategy
Someone who is trying to speed-read through this paper might take a quick glance at the data and see that the skin cream made more people’s rashes get better than those whose rashes got worse. On seeing this insight, they conclude by saying that the skin cream is effective and continue on their busy day.  

%Example Ratio Strategy
Someone else who thinks that I’m being tricky for some reason might look at this data and see the same insight as the previous person, but also notice that there’s another half of the data that the previous person ignored. Taking this data into account, they see that out of the people who didn’t use the skin cream, X\% of people got better, whereas of the people who did use the skin cream, only X\% of people got better. This leads the skeptical person to the conclusion that the skin cream is not effective.

%Heuristic is easy but leads to mistakes, ratio is hard but is more reliable
The first busy person in this example relied on a quick heuristic and went with the first conclusion that they found. However, this cursory calculation of the data did not result in the correct answer. The second skeptical person did get the correct answer, but in doing so, took more time and cognitive effort. We use this task and data because it’s easy to come to multiple interpretations based on what parts of the display you focus on.

%Motivation
Everyday, people use heuristic and rational thinking to come to conclusions. The conclusions could be from a range of XYZ to ZYX. When analyzing data, however, there are multiple ways to display data, which may result in different affordances. We are interested in two displays that are commonly used to display data: tables and bar graphs. We chose bar graphs because they are frequently found in the media and other daily uses. We hypothesize that patterns in bar graphs are 

%Study Overview
In this study, we use a cognitive reasoning task with the displays in \ref{teaser} to investigate the reasoning affordances in tables and bar graphs. Our findings suggest that people are more likely to use heuristics in bar graphs than in tables. We hypothesize the features of visual displays that afford heuristic strategies more than rational strategies.



==> Old_Files/old_exp_1.tex <==
\section{Experiment 1a: Skin Cream}
In a between-subject design experiment, we primed each participant with information about the company that produced the skin cream, randomized to be either positive or negative information. The positive prime described a successful company with a history of high-quality products, while the negative prime described an unsuccessful company that had violated federal health and safety policies. We intended this prime to bias participants into believing that the skin cream will be either effective or ineffective, to see if participants would be tempted to use a quicker, biased heuristic to make their judgment. 

%, resulting in confirmation bias, which would encourage people to take a look at the data more closely, enticing more``ratio" strategies. 
%so we can examine the effect of the tabular and bar displays at mitigating biases. This method of priming participants allowed us to randomly assign prior beliefs to participants, instead of relying on existing ones..

% By introducing a prime, we can investigate how belief interacts and bias problem solving with data with different strategies in this task. 

After reading the company description, participants viewed a skin cream data set, either as a tabular display (Figure \ref{teaser} top left) or a bar display (Figure \ref{abcd_skin}, but without the letters). %then viewed the same data displayed in either in a table or bar graph (as shown in Figure \ref{teaser}a, \ref{teaser}b), and 
Participants were asked whether using the skin cream made it more likely for rashes to get \textit{worse} or \textit{better}. They then typed their reasoning behind their decisions into an open-response text box while referencing the data they saw, labeled with %We also added an open-ended response for participants to explain the reasoning behind their decisions. For the open-ended responses, we asked participants to reference the cells by labels 
A, B, C, and D, as shown in Figure \ref{abcd_skin}. Participants  were instructed to explicitly refer to the cell labels as they described their strategies. %The letter labels were only shown for the open-ended responses, and not for the initial task. These labels allowed us to more easily determine which cells the participants were using for their calculations, and all coding was done blind to the trial's condition. % The table is adopted from previous work \cite{Kahan2017Motivated, Wasserman1990}. 

For the bar graph, we omitted numerical annotations (such as numeric value labels or numbers on the y-axis) to suppress verbal processing of the information, to ensure a purely visual comparison. These displays were counterbalanced by swapping the labels on the columns, such that for half of the participants the data suggested that the skin cream was effective. For the other half of the participants, the data suggested that the skin cream was ineffective. The experiment ended with participants self-reporting demographic information. 
%We coded trials as `congruent' if the correct conclusion from the data aligned with the prime (e.g., primed with good company and data shows effective skin cream), and `incongruent' otherwise (e.g., bad company but effective skin cream).


%The results also replicates an existing confirmation bias documented in psychology literature \cite{Kahan2017Motivated} and extend the investigation by examining the reasoning affordances of bar displays compared to table displays. 

\subsection{Participants}
Power analysis based on pilot data suggests that we would need at least 129 participants to achieve a 90\% power to detect an overall difference between response accuracy and data presentation format. %to leverage its more realistic setting for real-life decision making tasks than an undergraduate university setting \cite{Micallef2012}. 
We collected data from Amazon Mechanical Turk. In order to qualify for our study, participants needed to have a 95\% acceptance rate and be located in the United States. We implemented a series of quality checks to ensure that workers were paying attention (e.g., `How many years of experience of Computer Programming do you have? Please choose ``10+"  to show that you are paying attention.'). In addition to these attention check questions, we were able to track how long a person stayed on a page through Qualtrics. We used this to filter out workers who spent less than 10 seconds reading the descriptions of company, which was 2 paragraphs long. The mean completion time for reading these paragraphs was 33 seconds (median = 20 seconds).  %These stats include people who were excluded from later analysis.
We also excluded poor quality participants from analysis based on their open ended survey responses. %These may have been the most obvious to check for people that were not putting in effort into the survey. 
Low-quality responses ranged from off-topic answers to intelligible sentences. 56/59 of the workers who failed the timing check also failed the open-ended response check, suggesting that these two measures were both reliable at catching people who were not paying attention to the task. 

We iteratively sampled and excluded participants based on the above criteria from the experiment. We ended up with 138 participants due to an error in counterbalancing during experiment release so we randomly selected and excluded 9 participants to match the sample size of 129 derived from the power analysis ($M_{age}$ = 18.7(10.4), 47 female) such that 64 participants saw the bar chart and 65 participants saw the table display.

%\subsection{Hypotheses} 
%If people were being influenced by confirmation bias, we would expect the congruent condition (prime is that the company is good, data shows that the skin cream is effective) to have a higher rate of accuracy than the incongruent condition. For the incongruent condition, the first initial insight from a heuristic would be in line with the conclusion that they were primed, which also is the incorrect answer.

%In this study, we expect accuracy to be higher in the bar graph condition, as well as show a decrease in confirmation bias.

%A valid way to interpret the data presented in Figure \ref{stimuli} would be to focus on the proportion of crime increases and decreases under different circumstances. For example, under a handgun ban, 75/298 (25\%) cities displayed a decrease in crime, while with no ban, only 21/128 (16\%) of the cities had decreases in crime rates. For these particular data, once normalized with this strategy of converting numbers to ratios, it is clear that the ban is associated with reductions in crime.  \cx{we are still in the skin cream experiment, why is the example about crimes?}

%But for most people, that is a tough analytic task, requiring them to compare two ratios between pairs of numbers. It is instead tempting to use faster heuristics to interpret this data, which can lead to systematic biases \cite{kahneman1982}. Some people believe that banning concealed handguns will actually \textit{increase} crime, by removing a deterrent to criminal behavior. Thus, these people might focus only on the top row, where 223 cities that banned the weapons showed an increase in crime, compared to only 75 that showed a decrease. On the other hand, people that believe concealed carry will decrease crime might not accept that conclusion and interpret the data using the proportions of crime in each circumstance. This difficult task allows people to see the data from multiple perspectives which might justify either conclusion. These diverging conclusions illustrate confirmation bias.

%We hypothesized that the bar graph display would decrease confirmation bias. Both communicate the same ratios, though the tabular information conveys exact values while the bars do not. The bars may more intuitively convey the ratios among those values, and visual processing is typically faster and more powerful compared to text processing. 
 
%As we knew of no similar previous work for the visual depictions of the data, we did not have \textit{a priori} predictions for whether (a) accuracy would be higher or lower than in the tabular condition, or (b) confirmation bias would be stronger or weaker. 


%[Elsie] Note to self: Add confidence and timing?
%\subsection{Confidence Rating and Timing}

\subsection{Accuracy and Display Type}
\label{performance accuracy}

A logistic general linear model predicting accuracy with visualization display type suggested that participants were 3.72 times more likely to get the answer correct when they viewed the tabular display compared to the bar display ($Est = 1.31, SE = 0.30, p < 0.001$). See Figure \ref{results} for results.

\begin{figure}[tb]
 \centering 
 \includegraphics[width=\linewidth]{img/ABCD_skin.pdf}
 \caption{Participants were asked to describe their strategies using the A, B, C, D labels on the display. Letters were not present during the problem solving stage. This figure is a recreation of the stimuli with larger labels, and the actual stimuli shown is in supplementary materials. }
 \label{abcd_skin}
\end{figure} 


\subsection{Qualitative Coding}
Qualitative codes for possible strategies underwent several iterations before agreement on four categories: Ratio, Delta, Larger, and Other. The first and second author coded these responses, blind to condition. We initially attempted to organize strategies by which cells (A,B,C,D) a participant mentioned in their open ended response. For example, a common strategy was to compare cells A and C. However, we soon realized that it was also relevant to note the type of comparison that the participant was using. For example, it was important to note whether the participant was comparing whether B was overall larger than D, or whether they were comparing the ratio of B to D (3:1). Additionally, strategies could be complex, with people mentioning multiple comparisons, such as comparing \textit{both} A $>$ B and A $>$ C.

After many discussions between the authors, %coders, 
we decided to focus on the type of comparison instead of which cells were compared, and group responses into Ratio, Delta, Larger, and Other (see Figure \ref{strategy}). %This most closely reflects the underlying strategies of heuristic strategy (System 1) or rational strategy (System 2). 
One limitation of this coding structure is that it does not fully capture other points that a few participants mentioned, such as the differences in sample size. For example, one participant mentioned ``I did not think it was a very fair comparison as the totals in each group were different," which shows that the total amount of people in each group played a role in making a judgment. Another limitation to this coding structure is that it puts responses that only list one cell (e.g., only `A") into an Other category, because there is no comparison for a single cell. %There were also only participants that only listed 1 cell.

Another limitation for coding the open-ended responses was that even though we asked participants to refer to the cells in the data using the ABCD labels in Figure \ref{abcd_skin}, a few participants referred to the cells using the label names, forcing us to check which condition the participant was in before coding the response. %Fortunately, only a few participants did not follow the instructions in this way, and most used the ABCD labels. 


%Analysis
Discrepancies between coder ratings were discussed and resolved. These strategies were further coded into a binary factor - whether it is the correct ratio strategy, or a heuristic strategy. The following are examples of each strategy, as described by participants. See Figure \ref{strategy} for a sketched example of each strategy. 

% determined which the participants used the correct 'ratio' strategy for the skin cream effectiveness judgment task, and recorded the coding as a binomial variable --- a participant either used the ratio strategy, a heuristic strategy, or a strategy that did not fit into either of these. 
%\cm{[Could you share your coding scheme or your general definition for what the three coded-for strategies look like?]}


\textbf{Ratio}: Strategies were coded as Ratio if they mentioned ``proportions,'' ``percentages,'' or ``ratio'' and suggested a calculation of one of these values (e.g., for row 1) compared to another (e.g., compared to row 2). Some participants compared the rate of recovery of the people that used the skin cream (top row) to the rate of recovery of the people that did not use the skin cream (bottom row). Some participants used ratios not within the rows (as depicted in Figure \ref{strategy}), but instead within the columns. For example, they could compute the ratio of the people who ``got better'' was about 2:1, but the ratio of the people who ``got worse'' was greater than 3:1. 

\textit{Example Table Quote:}
Say the number of people who DID use the cream (A) is basically double that of those who DIDN'T (C), the number of people who's rash got worse (B) should be slightly more than doubled (D). Yet it's over 3x as big.

\textit{Example Bar Quote:}
In panel A, the people who used the cream had the rash get substantially worse. It was almost double of the people who did not use the cream (panel c).  The people who got better was almost 1/3 the number of the people who got worse using the cream (panel b).

\textbf{Delta}: Strategies were coded as Delta if they mentioned the difference between cells. This calculation is subtracting one cell from another cell (e.g., A-B). Participants commonly compared the deltas between two sets of cells (e.g., A-B is bigger than C-D). Note that this strategy is incorrect because subtraction is not a valid normalization operation for the present dataset, though it at least \textit{attempts} to normalize the data, in spirit. 

\textit{Example Table Quote:}
The difference between A and C was higher than the difference between B and D. Also, A is higher than B. This showed me that there were more people who got worse while using the cream than got better while using the cream and that more people got worse while using the cream than people who got worse while not using the cream. I think the people who got worse because of the cream is a more important result than the people that got better while using the cream. 

\textit{Example Bar Quote:}
Both of the answers were actually true. If you look at B and D you will see that people who used the cream also were more likely to get worse. If you look at A and C people who used the cream were also more likely to get better.  I chose my answer because the bigger difference in data looks to be A vs C.

\textbf{Larger}: Strategies were coded as Larger if the calculation was a greater than or less than comparison. This was the most common heuristic. Participants compared cells A and B, or A and C, or B and D, or a combination of these.

\textit{Example Table Quote:}
The count of people in table B is higher than the count of people in the table D.

\textit{Example Bar Quote:}
The bar in A is a lot higher than the bar in graph C.

\textbf{Other}: Any strategy that did not fit into the above categories but was still coherent was coded as Other. The following table example only mentions cell C and does not compare it with other cells or perform calculations. The participant in the bar example mentions the skin cream group and rashes that got worse, but it is unclear if they are making a comparison to anything. For the data in Experiment 1a in this category, two participants only mention one cell, two participants only describe the data without analyzing it, and three participants have responses that are unclear what they are referring to and/or comparing.

\textit{Example Table Quote:}
I wanted to choose that people got better by not using the cream as is conveyed in C. It wasn't a choice however. Between the two choices, patient getting better by using the cream seem to be a better response.

\textit{Example Bar Quote:}
Without knowing how many people are in each group, it appears the percentage of those who got worse are in the group that used the new skin cream. (Note that this participant appeared either to think that knowing the absolute value was critical or misunderstood that the bar represented a count. Experiment 1B redesigns the bar chart to minimize this latter potential misunderstanding)

We conduct a general logistic linear model predicting accuracy with a binary factor of the presence of the ratio strategy. The results suggest that using the ratio strategy significantly increases the likelihood of getting the correct answer by more than 4-fold ($Est = 1.44, SE = 0.38, p < 0.001$, $OR = 4.22$). Figure \ref{results} shows the percentage of participants who used these strategies (Ratio, Delta, Larger) in each condition.

\begin{figure*}[t]
 \centering 
 \includegraphics[width=\textwidth]{img/thumbnails.pdf}
 \caption{This table breaks down qualitatively coded strategies for each experiment condition. Across each row (study), the color-coded table cells represent the proportion of participants in that condition who used the strategy. The four general strategies are illustrated with blue sketches that depict examples of that comparison type. The comparisons shown are representative examples of the category, and not exhaustive.}
 \label{strategy}
\end{figure*} 

\subsection{Strategy Analysis}
\label{Experiment1DisplayStrategyAccuracy}
Why did participants perform worse overall when they viewed bar charts? We suspect that visualizing the information made certain patterns in the data more salient than others, affording different reasoning routines \cite{shah2011bar}. To examine this, we turn to the strategies each participants used to make their judgment. Figure \ref{results} shows the relationship between the strategy participants used and their task accuracy. 

We first investigated whether display type (bar or table) would elicit the right ratio strategy. A logistic regression model predicting the strategy participants used with visualization display type suggests that the tabular display more readily affords ratio strategies than the bar display ($Est = 1.60, SE = 0.38, p < 0.001, OR = 4.9$). We found the display type to be a significant predictor. Viewers were almost five times more likely to use the ratio strategy when viewing the tabular display.

%\subsection{Display Type and Strategy on Accuracy}
% We then conducted a post-hoc test that added the binary factor of the presence of the ratio strategy as a predictor, along with the interaction terms, to predict accuracy in addition to display type and congruency and their interaction, similar to section \ref{performance accuracy}. We started with a model that uses congruent bar displays with no ratio strategy as the baseline reference. This means bar graph displays are coded as 0 and tabular displays as 1. Congruent conditions are coded as 0 and incongruent conditions coded as 1. Participants that used the ratio strategy were coded as 1 and otherwise 0. As shown in Table \ref{odds1b}, the intercept represents the bar display congruent condition where participants did not use the ratio strategy. We can compare this intercept to the ratio variable (bolded in Table \ref{odds1b}), and see that, from this pair-wise comparison, the likelihood of participants getting the answers correct increases by 9.5 times when they use the ratio strategy in the congruent bar display condition. First we found that tables tend to afford more accurate judgment in this skin cream problem, especially when participants were primed in a congruent way that agrees with the data shown to them. \el{should I add a second graph that shows breakdown by conguency? If so, should I just include exp 1 data?} Then we found that using the right strategy significantly improves accuracy across all display and congruency conditions, especially so for the congruent conditions. 

%We then predicted whether using the ratio strategy would increase the odds of answering the reasoning question correctly. We used a similar logistic regression model predicting accuracy with whether the participant used the ratio strategy, and found that using the ratio strategy increase the odds of correctly answering the question 4.22 fold ($Est = 1.44, SE = 0.38, p < 0.001$). % Commented out redundant stats

We further constructed a logistic model predicting response accuracy with display type and whether the participant used the ratio strategy. We found a significant main effect of display type ($\chi^2$ = 5.33, $p = 0.021$), such that people who viewed the table display were more likely to reach the correct conclusion, and a significant main effect of strategy ($\chi^2$ = 8.07, $p = 0.0045$), such that people who used the ratio strategy were more likely to reach the correct conclusion, but no significant interaction ($\chi^2$ = 0.19, $p = 0.66$). 

Table \ref{exp1_OR2} shows the effect of strategy on accuracy. The odds ratio (OR) is interpreted as the likelihood of getting the correct answer given a unit change in the reference odds ratio. For example, the left of Table \ref{exp1_OR2} shows the odds ratio of answering the question correctly when participants viewed the bar chart display. The heuristic strategies (top row) are used as a reference. The odds of participants answering the question correctly is 0.26. When they use a ratio strategy instead, the odds of correctly answering the question is increased to 2.59 compared to using a heuristic strategy.

Overall, the additional consideration of strategy significantly captures more variance in predicting accuracy compared to only considering visualization display type ($Deviance = 8.26$, $p = 0.016$), suggesting that although participants were more likely to get the answer right when viewing the table display, using the normatively more correct ratio strategy also leads to more likely answering accurately.

\begin{table}[!h]
    \caption{Likelihood of a participant answering correctly when viewing the table vs. bar display, using or not using the ratio strategy. Left: using bar chart no ratio as baseline. Right: using table no ratio as baseline.}
    \begin{minipage}{.5\linewidth}
      \centering
          \begin{tabular}{llr}
  \newline \\
  \multicolumn{2}{c}{Bar chart} \\
   {\bf Strategy} & {\bf Odds Ratio} \\
  \hline 
 No ratio & 0.26 \\
 Ratio &  2.59 \\
     \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
       \begin{tabular}{llr}
  \newline \\
    \multicolumn{2}{c}{Table} \\
    {\bf Strategy} & {\bf Odds Ratio} \\
  \hline
 No ratio &  0.54\\
 Ratio &  3.71 \\
    \end{tabular}
    \end{minipage} 
        \label{exp1_OR2}
\end{table}

\subsection{Congruency}
Following the original reasoning paradigm in \cite{Kahan2017Motivated}, we also tested the effect of participants' prior beliefs on response accuracy. In this case, we imparted prior beliefs via a story prime that portrayed the company that produced the skin cream either in a positive or a negative way. We coded trials as `congruent' if the correct conclusion from the data aligned with the prime (e.g., primed with good company and data shows effective skin cream), and `incongruent' otherwise (e.g., bad company but effective skin cream).

We constructed a logistic model predicting response accuracy with congruency, visualization display type, and their interaction. We found a significant main effect of visualization display type($\chi^2$ = 12.38, $p = 0.00043$), replicating the findings from section \ref{Experiment1DisplayStrategyAccuracy} that people were more likely to answer the question correctly when viewing tables. We found no main effect of congruency ($\chi^2$ = 0.39, $p = 0.53$), such that overall, people were not more likely to answer the questions more correctly in situations where the correct answer is congruent with their belief, which is randomly imparted via a story prime. 

Interestingly, we found a significant interaction between congruency and visualization display type ($\chi^2$ = 11.65, $p = 0.0064$). In other words, for participants who viewed tabular displays, they were more likely to answer the question correctly if their prior belief is congruent with the data (e.g., participant read the story prime about a good company and the data showed an effective skin scream). For participants who viewed the bar displays, they was a surprising trend for participants to be more likely to answer the question correctly if their prior belief was \textit{incongruent} with data. While this result seems odd, we note that the overall accuracy for bar charts was very low overall, so that we cannot be confident of this result from the results of this experiment alone. To preview the results of the next experiment, this trend does not replicate in an improved design. 

Table \ref{exp1_congruency} shows the effect of belief-data congruency on accuracy. The left of Table \ref{exp1_congruency} shows the odds ratio of answering the question correctly when participants viewed the tabular display. The condition where the prior belief is congruent with data (top row) is used as a reference. The odds of participants answering the question correctly is 2.88. When their belief is incongruent with the data, the odds of correctly answering the question is decreased to only 24\% compared to when belief is congruent with the data.


In the Discussion below, we raise several possible critiques of the bar chart design used in Experiment 1a, which we address with Experiment 1b. 

%\cx{Additionally, several design flaws for the bar chart used in Experiment 1a lead to very low overall accuracy, so whether the effect of data-belief incongruency on improving accuracy remains unclear. To further investigate whether prior-belief affects how people reason beyond experimenter demand effects or poor design choices, we redesigned the bar chart in Experiment 1b and used a different scenario in Experiment 2 and recruited participants with certain prior beliefs.}

% edit table color
\begin{table}[!h]
    \caption{The effect of prior belief and visualization display type on accuracy. The odds ratio (OR) is interpreted as the likelihood of getting the correct answer given a unit change in the predictor. Left: tabular displays, with the condition where prior belief is congruent with data as reference. Right: bar displays, with the condition where prior belief is congruent with data as reference. }
    \begin{minipage}{0.5\linewidth}
     \centering
          \begin{tabular}{llr}
  \newline \\
       \multicolumn{2}{c}{Table} \\
       {\bf Congruency} & {\bf Odds Ratio} \\
  \hline 
 Congruent &  2.88\\
 Incongruent &  0.24 \\
     \end{tabular}
    \end{minipage}%
    \begin{minipage}{0.5\linewidth}
     \centering
       \begin{tabular}{llr}
  \newline \\
      \multicolumn{2}{c}{Bar} \\
  {\bf Congruency} & {\bf Odds Ratio} \\
  \hline
 Congruent & 0.16\\
 Incongruent &  3.69\\
     \end{tabular}
    \end{minipage}
        \label{exp1_congruency}
\end{table}

% \cx{A $\chi^2$ test of independence suggests an overall effect of data display type and accuracy ($\chi^2$ = 11.30, $p$ = $7.75e-4$, $Cramer's V$ = 0.30). A post-hoc comparison with Bonferroni adjustment suggests that participants were more likely to get the answer correct when they viewed the tabular display compared to the bar display ($p$ = 0.003). Further comparing the effect of congruency, for participants who viewed the tabular display, the ones in the congruent conditions were more likely to get the answer correct ($\chi^2$ = 5.90, $p$ = $0.015$, $Cramer's V$ = 0.29). Interestingly, for participants who viewed the bar display, they were less likely to get it correct in the congruent condition ($\chi^2$ = 5.39, $p$ = $0.020$, $Cramer's V$ = 0.29). Details can be found in the supplementary materials.}




\subsection{Discussion} 
Experiment 1a demonstrates that people are more likely to use an easier but incorrect heuristic strategy when data is presented in a bar display and are more likely to use a difficult but correct ratio strategy when data is presented in a tabular display (see Figure \ref{results}). %This suggests that the way the data is displayed has an effect on what type of strategy the participant uses, with Heuristics as a System 1 process and the Ratio strategy as a System 2 process. 

There is a relationship between strategy and accuracy, but it is of course not a one-to-one relationship. The heuristic strategy usually results in the wrong answer, but can sometimes lead to the correct answer by luck. For example, although heuristic users mostly compared A and C or A and B, a small subset of people compared B and D. This comparison that B is greater than D will lead to the correct answer, even if the participant's rationale is flawed. 

Some participants also mentioned multiple comparisons, such as mentioning B and D \textit{and} mentioning A and C. In this case, making both of these comparisons could lead the participant to come to either the right or wrong answer. One participant noted ``From the 2 options I felt that both were correct based on the graph shown. I noticed that A had a higher bar than C so I assessed that it meant more rashes got worse from using it than not using. I also saw that B had a bar higher than D which led me to believe the other option was correct, and that more people who used the cream got better than those who did not. These reasons are why I was not completely sure that my answer was correct, as I didn't expect both to be true. I am still not sure if both are true or if I was wrong."

The ratio strategy can also lead to an incorrect answer if the participant made a calculation error. For example, one participant reasoned: ``D is 5 times more likely to occur when patients did not use the skin screen in the group that wasn't treated vs B where patients were only 3 times more likely for the rash to worsen when being in the treatment group.'' This person should have made the calculation that D is 1/5 the size of C, instead they calculated that D was 5 times bigger than C. %due to calculation errors. %Since the problem does require multiple comparisons or calculations, it is possible that a mistake in one or more of these calculations could have resulted in the wrong answer.
Finally, in the bar condition, some participants noted that it was difficult to tell which ratio was larger: ``Without looking at actual numbers, it's hard to see what the ratio is between A and B, and if it's better or worse than the ratio between C and D." This participant is not able to accurately determine the ratio of each pair of numbers because they were not able to precisely compare the bar lengths. % to make the bar graph wider so it is easier to read. 

% After this analysis of interactions between strategy and accuracy, we decided to to focus our conclusions directly on strategy instead of how accurately that strategy was implemented, which differs from past work that relies on accuracy as a proxy for strategy \cite{Kahan2017Motivated}.

%We also find a difference between the congruent and incongruent conditions, suggesting that our priming influenced reasoning strategies. 

%We replicated and extended the finding from \cite{Kahan2017Motivated}, demonstrating that people suffer from confirmation bias when viewing tabular data, becoming more likely to choose the answer that is congruent to their belief, despite the belief being primed during the experiment. We found this not to be the case with bar visualizations. In a way, bar visualizations did mitigate confirmation bias, such that the primed belief was not a good predictor to whether they would get the answer correct or not. However, accuracy overall for bar visualization was much lower for both congruent and incongruent conditions.

%Further analysis revealed that this is likely due to the fact that participants were less likely to use the correct ratio strategy when they are viewing the bar visualization, and using the correct ratio strategy would boost their accuracy. 

% People who are primed with information that is congruent with the correct answer are more likely to choose that answer. People primed with incongruent information were less likely to be correct. This was true when the data were visualized as a table, replicating previous findings that people are systematically biased by their prior beliefs or group identities when doing this task. We also found that people are more likely to use correct ratio strategy in the tabular display than in the bar graph display. This slower and more difficult

While our results suggest that people were more likely to use the correct ratio strategy and more often answered correctly with the tabular display, the poor performance in the bar chart condition might also be driven by a misunderstanding due to the bar chart's design. The row axis labels may have misled participants to think the bar height reflected a percentage of people, rather than the absolute count of people. The lack of gridlines and the thin bar width design may have made bar length comparison difficult. %the sparse nature of the bar graph (e.g., no gridlines or axis markers) might have caused some participants to misunderstand what the bar graph depicted. 
For example, one participant reported ``People who did use the cream got better 90\% of the time in graph A,'' inaccurately interpreting the upper left cell as the percentage of everyone in a skin cream group who got better, instead of the raw count of people in the skin cream group who got better. To address this concern, Experiment 1b modifies the bar chart to make the design clearer and easier to read. 

%In order to untangle whether the disappearance of confirmation bias in the bar graph condition was due to participant confusion of the visualization, or visualizing the skin cream information actually reduces the prevalence of confirmation bias, we conducted a follow up experiment. In Experiment 2, we changed the Bar graph stimuli to include axis labels, in order to make it clear that the Bars represented number of people and not a percentage. We also made the bars wider and included grid lines behind the bars to make the bar graph easier and clearer to read.


\begin{figure*}[t]
 \centering 
 \includegraphics[width=\textwidth]{img/cb_stripes.pdf}
 \caption{Experiment 1 and Experiment 2 results. The left graph shows the percent of participants who were accurate for each condition. The Table condition had higher rates of accuracy. The right graph shows the percentage of participants for each type of strategy. Diagonal line patterns on each color indicates incorrect trials for that strategy. There is a higher percentage of ratio strategies for the tables than the bar charts. Most of the ratio strategies resulted in accurate trials, while most of the 'not ratio' strategies resulted in inaccurate trials. }
 \label{results}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Strategy, Congruency, Accuracy Rabbit Hole

%%%%% comment %%%%%%
\begin{comment}
\begin{table}[h]
\small
\renewcommand{\arraystretch}{1.3}
  \caption{\label{exp1accuracy} Logistic regression statistics model predicting odds of correctly judging skin cream effectiveness in the decision task, depending on whether the participants used the correct ratio strategy or not, using congruent bars without the ratio strategy as the baseline condition.}
  \begin{tabular}{lrrrlr}
  \newline \\
    {\bf Variable} & {\bf Ratio} & {\bf Est} & {\bf SE} & {\bf p-value} & {\bf OR} \\
  \hline 
  \textbf{intercept (congr. bars)} & no & -2.94 & 1.03 & 0.004** & 0.05\\
 display (congr. tables) & no & 2.54 & 1.37 & 0.065. & 12.67\\
 congr. (incongr. bars) & no & 2.37 & 1.11 & 0.032* & 10.69\\
  display*congr. (incongr. tables) & no & -2.98 & 1.55 & 0.055. & 0.05\\
 \textbf{ratio (congr. bars)} & yes & 2.25 & 1.25 & 0.071. & 9.50\\
 display*ratio (congr. tables) & yes & -0.75 & 1.61 & 0.642 & 0.47\\
 congr.ratio (incongr. bars) & yes & -1.68 & 1.49 & 0.261 & 0.19\\
 display*congr*ratio (incongr. tables) & yes & 1.50 & 1.95 & 0.441 & 4.49\\
    \end{tabular}
    \label{odds1b}
\end{table}


We performed similar post-hoc comparison for all other combinations using logistic regression by changing the baseline reference (intercept variable). Details are included in the supplementary materials, but a summary of the odds ratio comparisons is documented below. 

\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.3}
  \caption{\label{exp1accuracy} Change in odds ratio by using the ratio strategy for each display and congruency type. For example, for table display incongruent condition, using the ratio strategy would increase the likelihood of getting the right answer by 3.78 folds. }
  \begin{tabular}{llr}
  \newline \\
    {\bf Display} & {\bf Congruency} & {\bf Odds Ratio} \\
  \hline 
 bar & congruent & 9.50 \\
 bar & incongruent &  1.78 \\
 table & congruent &  4.50 \\
 table & incongruent &  3.78 \\
    \end{tabular}
    \label{odds1b}
\end{table}
\end{comment}

% We also conducted an ANOVA comparing regression models with whether the participant used the ratio strategy as a predictor to the model from section \ref{performance accuracy}, and found that it significantly captures more variance in predicting accuracy ($Deviance = 10.03$, $p = 0.039$).



==> Old_Files/old_exp_2.tex <==
\section{Experiment 2}

To generalize our results beyond the existing case study of skin cream effectiveness, Experiment 2 presents a new problem on gun control laws, and relies on existing opinions on gun control instead of a prime. In Experiment 1a and 1b, we primed participants to form an opinion about the skin cream company, to tempt them into using heuristic solutions. While we found strong differences in the type of reasoning used across bars and tables, we found weak and inconsistent effects of these prime manipulations. Experiment 2 simultaneously presents a new context to test the effects of congruency between a belief and a dataset on reasoning. 

%Additionally, we found an somewhat complicated effect of belief-data congruency on response accuracy. When people viewed tabular displays, those that were primed with information that is congruent with the correct answer are more likely to choose that answer, at least for the table condition. The opposite happened when they viewed bar charts, such that incongruent primes lead to higher accuracy. Although this seems to suggest that prior-belief can affect how participants reason in our task, it is unclear whether this effect would hold with participant's own beliefs that are held before they participate in the study. The story prime could have caused the participants to fall victim to 'experimenter demand effect', where they adapt their response to fit their anticipated experimenter's' expectations.

Participants viewed the same dataset either as a table display or the modified bar chart display, but framed in the context of gun control laws, as shown in Figure \ref{teaser}. The rows of the table represent two groups: one consisting of cities that had recently enacted bans on concealed weapons and another that had cities with no such bans. In each row, the left column shows %there is 
the number of cities that experienced decreases in crime and the right column shows those that experienced increases in crime. %in the next year. The design remains identical to Experiment 1a and 1b.

\subsection{Participants}
Participants were recruited from Amazon's Mechanical Turk following the same exclusion criteria as before. Because people already have prior beliefs on the effectiveness of gun control laws, we did not assign people to a priming condition and removed the exclusion check for time spent reading the prime. At the end of the session, we asked about their political affiliations and their operational beliefs about gun control laws. Specifically, we asked them to rate how much they agree with the statement ``greater gun restriction laws are necessary to reduce violence'' on a scale from 1 (strongly disagree) and 7 (strongly agree). This self-reported information was used to identify people as being more likely to either believe that stricter gun control laws will reduce (anti-gun) or increase (pro-gun) crime. 

Participants then viewed data displayed either in a table or bar chart (as shown in Figure \ref{teaser} (bottom row), and were asked whether a ban on concealed carrying concealed weapon made it more likely for crime to \textit{increase} or \textit{decrease}. Their judgment on whether the ban on concealed carry was effective or not was coded as accurate if it was supported by the data they viewed. Similar to Experiment 1a and 1b, they then explained the strategies behind their decisions.
%Then, they reported how confident they were with their answer on a scale of 1 to 5. \cx{do we still want to talk about the confidence thing?} We also added an open-ended response for participants to explain the strategies behind their decisions. 

Again, displays were counterbalanced such that for half of the participants the data suggested that the ban on concealed carry was effective. For the other half of the participants, the data suggested that the ban on concealed carry was ineffective, by swapping the labels on the columns. After applying exclusion criteria, we were left with 204 participants ($M_{age}$ = 21.08(12.62), 104 female), 105 of which viewed the bar chart and 99 viewed the table. 

%\subsection {Confidence and Timing}


\subsection{Accuracy and Display Type}
\label{performance accuracy}
Similar to the skin-cream experiment, participants were more likely to respond correctly when the data was presented in a table. We again constructed a logistic general linear model predicting accuracy with display type (bar chart or table display), and found the table display increased the odds of participants answering the question correctly 2.70 folds ($Est = 0.99, SE = 0.31, p = 0.0013, OR = 2.70$).


% Qual Coding
\subsection{Qualitative Coding of Strategies}
We again coded the strategies each participant used to make their judgment. The coding structure was the same as Experiment 1. Some example quotes are included below.

\textbf{Ratio}: 

\textit{Example Table Quote: }
Total cities that did ban by adding A + B = 298 while cities that did not ban (C + D) was 128. For those that did ban, about 1/4 saw crime rates decrease. For those that did not, only 1/6 saw a decrease. Other variables were surely in play but based on that alone, I feel the ban did help to decrease crime overall.

\textit{Example Bar Quote: }
I felt that comparing A vs C and B vs D the rations showed that A was about double the figure of C.  Whereas B was about three times higher than D showing that banning handguns increased crime somewhat.  It would seem like the obvious choice did not have the desired effect.

\textbf{Delta}:

\textit{Example Table Quote: }
I attempted to calculate the net decrease in crime for cities that did and did not ban carrying concealed handguns in public. For cities that did choose to ban concealed guns I got 148 (A - B). For cities that did not choose to ban concealed guns I got 86 (C - D). The net decrease was greater in cities that banned concealed guns.

\textit{Example Bar Quote: }
I subtracted the right columns (B and D) from the left columns (A and C). The one with the smaller remaining number of cities was the option that worked best. This is because it means they had the lowest number of cities with a net increase in crime.

\textbf{Larger}:

\textit{Example Table Quote: }
I looked at mostly A and C. From there is where I concluded. I feel like I got it right.

\textit{Example Bar Quote: }
A. I used choice A because the number of crimes have jumped up too high and is almost to the top of the chart. Comparative to the other charts, there is some increase in crime, but the rate is exponentially more in choice A. The decrease in crime in choice B shows that it doesn't compare to the increase in crime in choice A. 

\textbf{Other}:

\textit{Example Table Quote: }
It is clear that banning guns on law abiding citizen will only increase crime. Only because criminals don't get their guns legally only on the black market. It doesn't help anyone to ban handguns.

\textit{Example Bar Quote: }
You can clearly see what's going on in A. There is a huge spike that shows crime decreased. Therefore, if you ban the guns, crime will decrease. People don't have guns and there will be less violence. 
\\


\subsection{Strategy Analysis}
% when is the participant more likely to use the ratio strategy?
In Experiment 1 we found that tables were more likely to elicit ratio strategies. We conducted a similar logistic regression model here predicting whether the participant used the ratio strategy using display type as the predictor. Again, display type was a significant predictor ($\chi^2$ = 12.52, $p < 0.001$, $OR = 3.07$), such that the odds of participants using the correct ratio strategy is increased 3 folds when they solved the problem with the tables compared to the bar chart. 

% is the ratio strategy more accurate?
Previously we also found that using the correct ratio strategy also leads to higher likelihood of answering the question correctly. To see if this generalizes to this new scenario, we conducted a general logistic linear model predicting accuracy with a binary factor of whether the participant used the ratio strategy. The results, again, suggest that using the ratio strategy significantly increases the odds of getting the correct answer ($\chi^2$ = 52.44, $p < 0.001$, $OR = 11.31$). 

% interaction between ratio strategy and display on accuracy
Previously, in Experiment 1b, we also found that although participants were overall more likely to use the ratio strategy when they viewed the tabular display, some still used the ratio strategy when viewing the bar chart. For everyone that used the ratio strategy, they were more likely to answer the question correctly when they viewed the modified bar chart compared to the table (see section \ref{1bStrategyAnalysis}).

To see if this finding generalizes to this new scenario, we constructed a similar logistic model where we predicted response accuracy with display type and whether the participants used a ratio strategy in this new context. We found a significant main effect of strategy ($\chi^2$ = 44.73, $p < 0.001$), such that participants who used the ratio strategy were more likely to reach the correct conclusion. We also found a trendingly significant main effect of display type ($\chi^2$ = 3.08, $p = 0.079$), such that participants who viewed the data in a tabular display were more likely to reach the correct conclusion, but no interaction between the two ($\chi^2$ = 1.84, $p = 0.17$).

In this experiment, we see that people were more likely to answer correctly by using the ratio strategy. But for those that used the ratio strategy, the odds of answering the question correctly is higher when participants viewed the tabular display, compared to the bar chart. There is a discrepancy between this finding, and that in Experiment 1b (such that the direction of the \textit{interaction term} of ratio strategy crossed with visualization display type is different). We further reflect on this in section \ref{discussion}.  Table \ref{exp2_OR} shows the odds ratio of participants getting the answer more correctly for the two display types, either with or without using the ratio strategy. The left table uses tabular display without the ratio strategy as reference, while the right table uses bar chart without the ratio strategy as reference.

\begin{table}[!h]
       \small
    \caption{Likelihood of a participant answering correctly when viewing the table (left) vs. bar (right) display, with or without using the ratio strategy. The condition where people did not use the ratio strategy is used as the reference.}
    \begin{minipage}{.5\linewidth}
      \centering
          \begin{tabular}{lr}
  \newline \\
    \multicolumn{2}{c}{Table} \\
    {\bf Strategy} & {\bf Odds Ratio} \\
  \hline 
No ratio & 0.26 \\
 Ratio &  15.67 \\
     \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
       \begin{tabular}{lr}
  \newline \\
     \multicolumn{2}{c}{Bars} \\
     {\bf Strategy} & {\bf Odds Ratio} \\
  \hline
 No ratio &  0.19 \\
  Ratio &  5.71 \\
    \end{tabular}
    \end{minipage} 
        \label{exp2_OR}
\end{table}


% Congruency
\subsection{Congruency}
Although not the focus of the study, we observed a tendency for participants to more often answer the reasoning question correctly when the data is congruent with their belief in Experiment 1 if they viewed tables. We now examine whether this effect of data-belief congruency on improving accuracy generalizes to the new gun control legislation scenario, where belief is not endowed by a randomized prime, but instead is a pre-existing belief for the participant.

We categorized participants based on their self-reported stance on gun restriction laws into pro-gun restriction laws, neutral, and anti-gun restriction laws. The participants whose belief aligns with the data they viewed (e.g., a pro-gun restriction law participant viewing data showing banning concealed weapon \textit{reduced crime rates}) were coded as congruent, while those whose belief oppose the data they viewed (e.g., a pro-gun restriction law participant viewing data showing banning concealed weapon \textit{increase crime rates}) were coded as incongruent. Participants with neutral attitudes towards gun-restriction laws were coded as neutral. 

There were very few participants who held neutral attitude towards gun-restriction laws (9.8\%). In total, 18.1\% of the participants held a strong congruent belief (e.g., they are pro-gun restriction laws and the experiment stimulus data suggests gun restriction laws is effective), 11.8\% held medium congruent belief, 18.1\% held weak congruent belief, 12.7\% held medium incongruent belief, 9.8\% held weak incongruent belief, and 19.6\% held strong incongruent belief. See the comprehensive breakdown by display type and strategy used in the supplementary materials. We assigned numerical values to this spectrum, where 1 represents a strong incongruent belief, and 7 represents a strong congruent belief. We will refer to these values as belief-data congruency.

We constructed a logistic general linear model predicting accuracy with belief-data congruency, display type and their interaction. There was a significant main effect of display type, such that participants were more likely to answer the question correctly when they viewed the table display ($\chi^2$ = 10.14, $p$ = $0.0014$). We found a trendingly significant effect of congruency on accuracy ($\chi^2$ = 3.63, $p$ = $0.057$), such that higher belief-data congruency trendingly leads to higher odds of correctly answering the question. There was no significant interaction between display and congruency ($\chi^2$ = 0.30, $p$ = $0.58$). While the effect of belief-data congruency on increasing accuracy seems trendingly significant, we hesitate to draw strong conclusions from them. %For example, for those that viewed the bar chart, as shown on the right column in Figure \ref{exp2_congruency}, a higher percentage of participants answered the question correctly when their belief is 'medium congruent' with the data, compared to those whose belief is strongly congruent with the data. We reflect on this further in section \ref{discussion}}. 

% \begin{figure}[h!]
%  \centering 
%  \includegraphics[width=\linewidth]{img/Exp2Congruency.jpg}
%  \caption{The effect of belief-data congruency on accuracy for table and bar chart. Generally, stronger belief congruent with data leads to higher accuracy, but the result is especially noisy for bar chart.} %\el{Is there a reason why Weak is underlined?}}
%  \label{exp2_congruency}
% \end{figure}

\subsection{Discussion} 
For Experiment 2, we found that tables again more readily afforded the correct ratio strategy compared to %more than 
the bar chart. This suggests that this effect that we found for Experiment 1 and 2 holds for different contexts. %, with the odds ratio for both being that tables are 3 times more likely than bar charts to produce the ratio strategy.
As a result, participants were more likely to reach the correct answer when solving the problem with a tabular display compared to bar chart. %, since they were more likely to use the correct ratio strategy. 
This also replicates the findings of Experiment 1.

Additionally, we found that some participants used ideological justifications for their decision instead of, or in addition to, referencing the data. For example, one participant mentioned ``The data shows that cities that did ban the handguns showed an increase in crime. This is likely due to rights being taken away." This shows that the context did have an effect on reasoning, with prior beliefs consciously (and potentially unconsciously) influencing what parts of the data people attend to and favor in their judgments. This suggests that participants are driven to draw conclusions from data that are consistent with their beliefs. However, this effect remains small and inconsistent across our experimental conditions. Although not the focus of the study, we discuss future directions that could investigate the effect of belief-congruency on data reasoning.


==> TODO.tex <==

unify how you refer to bar vs. tabular throughout the paper


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

